Degeneration-Tuning: Using Scrambled Grid shield Unwanted Concepts from Stable Diffusion

Owing to the unrestricted nature of the content in the training data, large text-to-image diffusion models, such as Stable Diffusion (SD), are capable of generating images with potentially copyrighted or dangerous content based on corresponding textual concepts information. This includes specific intellectual property (IP), human faces, and various artistic styles. However, Negative Prompt, a widely used method for content removal, frequently fails to conceal this content due to inherent limitations in its inference logic. In this work, we propose a novel strategy named \textbf{Degeneration-Tuning (DT)} to shield contents of unwanted concepts from SD weights. By utilizing Scrambled Grid to reconstruct the correlation between undesired concepts and their corresponding image domain, we guide SD to generate meaningless content when such textual concepts are provided as input. As this adaptation occurs at the level of the model's weights, the SD, after DT, can be grafted onto other conditional diffusion frameworks like ControlNet to shield unwanted concepts. In addition to qualitatively showcasing the effectiveness of our DT method in protecting various types of concepts, a quantitative comparison of the SD before and after DT indicates that the DT method does not significantly impact the generative quality of other contents. The FID and IS scores of the model on COCO-30K exhibit only minor changes after DT, shifting from 12.61 and 39.20 to 13.04 and 38.25, respectively, which clearly outperforms the previous methods.

==> content/1_abs.tex <==
\section{abstract}
Due to the unrestricted nature of the content in the training data, large text-to-image diffusion models, such as Stable Diffusion (SD), can generate images with potentially copyrighted or dangerous content based on corresponding textual concepts information. This includes specific intellectual property (IP), human faces, and various artistic styles. However, the Negative Prompt, one of the most widely used method for content removal, always fails to conceal this content due to its inherent limitations in inference logic. In this work, we produce a novel strategy called \textbf{Degeneration-Tuning(DT)} to shield contents of unwanted concepts from SD weights. By utilizing Scrambled Grid to reconstruct the correlation between undesired concepts and their corresponding image domain, we steer SD to generate meaningless content when such textual concepts are provided as input. Since this adaptation occurs at the level of the model's weights, the SD, after DT, can be grafted to other conditional diffusion frameworks like ControlNet to shield unwanted concepts. % Moreover, these effects also cannot be circumvented even if the parameters of this model has been attacked or leaked. 
In addition to qualitatively showcasing the effectiveness of our DT method in protecting various types of concepts, the quantitative comparison of the SD before and after DT indicates that DT method does not significantly impact the generative quality of other contents. The FID and IS scores of the model on COCO-30K exhibit only slight changes after DT, shifting from 12.61 and 39.20 to 13.04 and 38.25, respectively. The results of continual DT suggest that although DT remains effective in scenarios requiring shielding unwanted concepts continuously, challenges still persist. The FID and IS on COCO-30K in continual DT change from 12.63 and 38.77 to 15.32 and 35.71.



















==> content/7_experiments_analysis.tex <==
\section{Analysis and Ablation}
\subsection{add original parameters}

\subsection{positive and negative samples proportion}

\subsection{without None prompt}

\subsection{add some cc12m captions}

\subsection{size of scrambled grid}



















